The Einstein@Home Gamma-Ray Pulsar Survey II. Source Selection, Spectral Analysis and Multi-wavelength Follow-up

We report on the analysis of 13 gamma-ray pulsars discovered in the Einstein@Home blind search survey using Fermi Large Area Telescope (LAT) Pass 8 data. The 13 new gamma-ray pulsars were discovered by searching 118 unassociated LAT sources from the third LAT source catalog (3FGL), selected using the Gaussian Mixture Model (GMM) machine learning algorithm on the basis of their gamma-ray emission properties being suggestive of pulsar magnetospheric emission. The new gamma-ray pulsars have pulse profiles and spectral properties similar to those of previously-detected young gamma-ray pulsars. Follow-up radio observations have revealed faint radio pulsations from two of the newly-discovered pulsars, and enabled us to derive upper limits on the radio emission from the others, demonstrating that they are likely radio-quiet gamma-ray pulsars. We also present results from modeling the gamma-ray pulse profiles and radio profiles, if available, using different geometric emission models of pulsars. The high discovery rate of this survey, despite the increasing difficulty of blind pulsar searches in gamma rays, suggests that new systematic surveys such as presented in this article should be continued when new LAT source catalogs become available.

==> radio_followup.tex <==
\begin{deluxetable*}{llcccrrr}[p]
	
	\tablecaption{\label{t:radio_followup} Follow-up radio observations}%
	\tablecolumns{8}
	\tablehead{
		\colhead{PSR} &
		\colhead{Reciever}&
		\colhead{Central frequency (MHz)}&
		\colhead{Bandwidth (MHz)}&
		\colhead{$t_{int}$ (s)}&
		\colhead{$S$(${\mu}Jy$)}&
		\colhead{Offset (')}&
		\colhead{Ref}
	}
	\startdata
	\textbf{J0002+6216}	& Eff-L1&1360&140&7200 &20&0&this work\\
	J0359+5414 	& Eff-L1 		&1360&140&7200 &30&0&this work\\
	...			& Eff-L1 		&1360&140&7200 &30&0&this work\\
	\textbf{J0631+0646} & Eff-L1&1360&140&7200 &30&0&this work \\
	... 		& AO-327 		&327&68 &4200 &*28&0&this work \\
	J1057-5851	& ? 			&?	 &?  &?    &? &? &?\\
	J1105-6037 	& ? 			&?	 &?  &?    &? &? &?\\
	J1350-6225 	&Parkes L-band 	&1390&256&4320 &?	&?&HTRU?\\
	... 		&Parkes 10cm	&?	 &?	 &26280&?	&?&HTRU?\\
	... 		&Parkes 20cm	&?	 &?	 &29880&?	&?&HTRU?\\
	J1528-5838 	&Parkes L-band	&1390&256&4320 &?	&?&HTRU?\\
	J1623-5005  & ? 			&?	 &?  &?    &? &? &?\\
	J1624-4041	& GMRT607		&607 &?	 &?	   &?	&?&?\\	
	...			& GMRT607		&607 &?	 &?	   &?	&?&?\\
	...			& GMRT306		&306 &?  &?    &?	&?&?\\
	...			& Parkes		&1390&256&3600 &200&1.13&Camilo et al.\\
	...			& Parkes		&1390&256&3600 &200&1.13&Camilo et al.\\
	J1650-4601  & ? 			&?	 &?  &?    &? &? &?\\
	J1827-1446 	& Eff-L1 		&1360&140&7200 &30	&0&this work\\
	... 		& Eff-L1 		&1360&140&7200 &30	&0&this work\\
	J1844-0346	& Eff-L1 		&1360&140&7200 &30	&0&this work\\
	J2017+3625 	& Eff-L1 		&1360&140&7200 &30	&0&this work\\
	... 		& Eff-L1 		&1360&140&7200 &30	&0&this work\\
	... 		& AO-L-wide 	&1420&600&2000 &22	&0&this work\\
	%	...			& FR606			&150&N/A&21600&?\\
	\enddata
	\tablecomments{Column 2-5, listed the telescope reciever used, central frequency, band width and exposure time respectivly. In column 6, therioical flux density were calculated using the modified radiometer equation \citep[Equation A1.22,][]{lorimer2005handbook} based on the central frequency, band width and exposure time, flux density with asterisk are flux density extrapolate from 327 Mhz to 1.4 Ghz assuming a spectral index of $\alpha$ = -1.7.}
	%	To be completed\\
	\end{deluxetable*}
	

==> radio_followup_v2.tex <==
\begin{deluxetable*}{lcccccccc}[p]
	
	\tablecaption{\label{t:radio_follow_up} Definition of Radio Observation Codes}%
	\tablecolumns{9}
	\tablehead{
		\colhead{Target} &
		\colhead{Obs Code}&
		\colhead{Date}&
		\colhead{$t_{obs}$}&
		\colhead{R.A.}&
		\colhead{Decl.}&
		\colhead{Offest}&
		\colhead{$T_{sys}$}&
		\colhead{$S_{min}$}\\
		\colhead{PSR}&
		\colhead{}&
		\colhead{}&
		\colhead{(min)}&
		\colhead{(J2000)}&
		\colhead{(J2000)}&
		\colhead{arcmin}&
		\colhead{K}&
		\colhead{$\mu$Jy}
	}
	\startdata
J0002+6216	&	GBT-Sband	&	2013-02-28	&	28	&	0.668	&	62.279	&		&		&		\\
J0359+5414	&	Eff-L 	&	2010-07-17	&	60	&	59.881	&	54.196	&		&		&		\\
J0359+5414	&	Eff-L	&	2010-05-25	&	32	&	59.899	&	54.178	&		&		&		\\
J0359+5414	&	GBT-Sband	&	2012-11-17	&	40	&	59.901	&	54.216	&		&		&		\\
J0359+5414	&	GBT-Sband	&	2013-03-17	&	7x7	&	59.901	&	54.216	&		&		&		\\
J0631+0646	&	AO-327	&	2015-03-15	&	70	&	97.968333	&	6.770556	&		&		&		\\
J0631+0646	&	AO-Lwide	&	2015-06-14	&	69	&	97.968333	&	6.770556	&		&		&		\\
J1057-5851	&	Parkes	&		&	75	&		&		&		&		&		\\
J1057-5851	&	Parkes	&	2015-08-05	&	70	&	164.288917	&	-58.853056	&		&		&		\\
J1057-5851	&	Parkes	&	2015-08-06	&	51	&	164.288917	&	-58.853056	&		&		&		\\
J1105-6037	&	Parkes	&	2015-08-05	&	70	&	166.252	&	-60.621	&		&		&		\\
J1105-6037	&	Parkes	&	2015-08-06	&	60	&	166.252	&	-60.621	&		&		&		\\
J1350-6225	&	Parkes-AFB	&	2010-11-19	&	145	&	207.400	&	-62.400	&		&		&		\\
J1350-6225	&	Parkes-BPSR	&	2010-11-19	&	144	&	207.400	&	-62.400	&		&		&		\\
J1350-6225	&	Parkes	&	2015-09-05	&	433	&	207.685	&	-62.429	&		&		&		\\
J1350-6225	&	Parkes	&	2015-09-13	&	500	&	207.685	&	-62.429	&		&		&		\\
J1528-5838	&		&		&		&		&		&		&		&		\\
J1623-5005	&	Parkes-BPSR	&	2010-11-19	&	144	&	245.700	&	-50.100	&		&		&		\\
J1623-5005	&	Parkes-AFB	&	2010-11-19	&	88	&	245.700	&	-50.100	&		&		&		\\
J1624-4041	&	Parkes-AFB	&	2010-07-18	&	120	&	246.013	&	-40.716	&		&		&		\\
J1624-4041	&	Parkes-AFB	&	2010-07-26	&	120	&	246.013	&	-40.716	&		&		&		\\
J1624-4041	&	Parkes-AFB	&	2010-11-12	&	60	&	246.013	&	-40.716	&		&		&		\\
J1624-4041	&	GMRT-610	&	2011-02-15	&	60	&	246.016	&	40.689	&		&		&		\\
J1624-4041	&	GBT-S	&	2009-12-23	&	30	&	246.025	&	-40.680	&		&		&		\\
J1624-4041	&	 Parkes-AFB	&	2009-12-02	&	120	&	246.026	&	-40.680	&		&		&		\\
J1624-4041	&	Parkes-AFB	&	2012-07-12	&	60	&	246.038	&	-40.673	&		&		&		\\
J1624-4041	&	Parkes-AFB	&	2012-12-17	&	60	&	246.038	&	-40.673	&		&		&		\\
J1624-4041	&	GMRT-322	&	2012-07-12	&	60	&	246.038	&	-40.673	&		&		&		\\
J1650-4601	&	Parkes-BPSR	&	2010-11-21	&	144	&	252.700	&	-46.100	&		&		&		\\
J1650-4601	&	Parkes-AFB	&	2010-11-21	&	139	&	252.700	&	-46.100	&		&		&		\\
J1827-1446	&	GBT-820	&	2014-04-21	&	35	&	276.834	&	-14.767	&		&		&		\\
J1844-0346	&	Eff-L	&	2010-05-15	&	32	&	281.064	&	-3.713	&		&		&		\\
J1844-0346	&	Eff-L 	&	2010-07-30	&	60	&	281.091	&	-3.701	&		&		&		\\
J1844-0346	&	Eff-L 	&	2010-07-31	&	60	&	281.091	&	-3.701	&		&		&		\\
J1844-0346	&	GBT-Sband	&	2012-11-17	&	22	&	281.109	&	-3.756	&		&		&		\\
J2017+3625	&	AO-ALFA	&	2015-05-11	&	20	&	304.476	&	36.39	&		&		&		\\
J2017+3625	&	AO-327	&	2015-06-24	&	15	&	304.483	&	36.459	&		&		&		\\
J2017+3625	&	AO-327	&	2015-06-25	&	15	&	304.483	&	36.459	&		&		&		\\
J2017+3625	&	LOFAR-HBA	&	2015-01-23	&	385	&		&		&		&		&		\\
J2017+3626	&	AO-327	&	2015-11-16	&	28	&	304.483	&	36.419	&		&		&		\\
J2017+3625	&	AO-Lwide	&	2015-11-17	&	33	&	304.483	&	36.419	&		&		&		\\
J2017+3625	&	Nancay-L	&	2010-05-05	&	60	&	304.450	&	36.438	&		&		&		\\
J2017+3625	&	GBT-820	&	2011-01-15	&	45	&	304.490	&	36.460	&		&		&		\\
J2017+3625	&	GBT-S	&	2010-05-13	&	60	&	304.496	&	36.422	&		&		&		\\
	\enddata
	\tablecomments{}
	%	To be completed\\
	\end{deluxetable*}
	

==> ranked_sources.tex <==
\clearpage 

\LongTables

\begin{deluxetable*}{lllrrrrrrr}[p]		
	
	\tablecaption{\label{t:source_list} Ranked Source List}
	\tablecolumns{10}
	\tablehead{
		\colhead{3FGL Name}&
		\colhead{Pulsar Name}&
		\colhead{2FGL Name}& 
		\colhead{VI}&
		\colhead{$TS_{curve}$}&
		\colhead{$TS_{cutoff}$}&
		\colhead{$E_{cutoff}$}&
		\colhead{$\Gamma$}&
		\colhead{TS}&
		\colhead{Class}\\
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{(GeV)}&
		\colhead{}&
		\colhead{}&
		\colhead{}
	}
	\startdata
	3FGL J1745.3$-$2903c			&	...				&	...					&	48.4	&	275.2	&	378.7	&	2.2	&	1.4	&	3407	&	...	\\
	3FGL J1746.3$-$2851c			&	...				&	2FGL J1746.6$-$2851c&	57.1	&	113.0	&	364.7	&	4.0	&	1.5	&	2373	&	pwn	\\
	3FGL J2017.9$+$3627				&	PSR J2017$+$3625&	2FGL J2018.0$+$3626	&	39.9	&	179.3	&	198.9	&	1.9	&	1.4	&	1876	&	...	\\
	3FGL J1839.3$-$0552				&	...				&	...					&	37.4	&	83.7	&	135.1	&	2.3	&	1.2	&	714		&	...	\\
	3FGL J1906.6$+$0720$^\dagger$	&	PSR J1906$+$0720&	2FGL J1906.5$+$0720	&	41.7	&	87.9	&	68.6	&	7.0	&	2.0	&	1580	&	...	\\
	3FGL J1910.9$+$0906$^\dagger$	&	...				&	2FGL J1911.0$+$0905	&	52.3	&	53.2	&	17.4	&	41.7&	2.1	&	4790	&	snr	\\
	3FGL J1636.2$-$4734				&	...				&	...					&	54.6	&	106.0	&	47.1	&	7.1	&	1.9	&	1180	&	snr	\\
	3FGL J1848.4$-$0141				&	...				&	2FGL J1848.2$-$0139c&	52.6	&	109.0	&	13.8	&	9.8	&	2.5	&	1457	&	...	\\
	3FGL J1405.4$-$6119$^\dagger$	&	...				&	2FGL J1405.5$-$6121	&	43.9	&	61.1	&	19.7	&	8.2	&	2.1	&	1671	&	...	\\
	3FGL J1111.9$-$6038$^\dagger$	&	...				&	2FGL J1112.1$-$6040	&	46.7	&	81.4	&	58.5	&	10.4&	1.9	&	3624	&	spp	\\
	3FGL J1748.3$-$2815c			&	...				&	...					&	34.1	&	77.4	&	68.6	&	4.7	&	1.4	&	489		&	...	\\
	3FGL J1622.9$-$5004$^\dagger$	&	PSR J1623$-$5005&	2FGL J1622.8$-$5006	&	54.4	&	72.4	&	73.3	&	8.0	&	1.6	&	891		&	...	\\
	3FGL J0223.6$+$6204$^\dagger$	&	...				&	2FGL J0224.0$+$6204	&	41.8	&	86.3	&	182.6	&	1.8	&	1.5	&	1089	&	...	\\
	3FGL J1823.2$-$1339$^\dagger$	&	...				&	2FGL J1823.1$-$1338c&	47.5	&	29.7	&	47.4	&	9.0	&	1.9	&	1004	&	...	\\
	3FGL J1745.1$-$3011				&	...				&	...					&	59.7	&	92.7	&	88.8	&	0.6	&	0.4	&	459		&	spp	\\
	3FGL J1800.8$-$2402$^\dagger$	&	...				&	2FGL J1800.8$-$2400	&	46.7	&	36.4	&	21.3	&	11.3&	1.7	&	575		&	...	\\
	3FGL J1749.2$-$2911				&	...				&	...					&	41.8	&	50.9	&	43.6	&	1.6	&	1.3	&	265		&	...	\\
	3FGL J1306.4$-$6043$^\dagger$	&	...				&	2FGL J1306.2$-$6044	&	35.7	&	65.9	&	42.6	&	8.6	&	1.7	&	1108	&	...	\\
	3FGL J1104.9$-$6036$^\dagger$	&	PSR J1105$-$6037&	2FGL J1104.7$-$6036	&	43.1	&	77.4	&	64.6	&	3.6	&	1.7	&	769		&	...	\\
	3FGL J0634.1$+$0424				&	...				&	...					&	42.9	&	123.3	&	60.2	&	1.8	&	2.2	&	1421	&	...	\\
	3FGL J1552.8$-$5330				&	...				&	...					&	46.4	&	56.6	&	50.3	&	1.8	&	1.0	&	210		&	...	\\
	3FGL J1747.0$-$2828				&	...				&	...					&	90.6	&	159.7	&	135.3	&	2.5	&	1.8	&	1676	&	...	\\
	3FGL J1650.3$-$4600				&	PSR J1650$-$4601&	2FGL J1650.6-4603c	&	55.1	&	54.6	&	55.0	&	4.8	&	1.8	&	897		&	...	\\
	3FGL J2323.4$+$5849				&	...				&	2FGL J2323.4$+$5849	&	40.1	&	62.4	&	39.1	&	26.4&	1.6	&	2568	&	snr	\\
	3FGL J1625.1$-$0021$^\dagger$	&	...				&	2FGL J1625.2$-$0020	&	37.3	&	104.3	&	201.4	&	1.9	&	0.8	&	1778	&	...	\\
	3FGL J1714.5$-$3832				&	...				&	2FGL J1714.5$-$3829	&	68.8	&	39.3	&	23.3	&	14.7&	2.2	&	2649	&	snr	\\
	3FGL J1857.9$+$0210$^\dagger$	&	...				&	2FGL J1857.6$+$0211	&	50.6	&	42.8	&	50.5	&	3.2	&	1.9	&	601		&	...	\\
	3FGL J1056.7$-$5853$^\dagger$	&	PSR J1057$-$5851&	2FGL J1056.0$-$5853	&	35.7	&	88.2	&	126.1	&	1.1	&	1.5	&	596		&	...	\\
	3FGL J1026.2$-$5730				&	...				&	...					&	50.4	&	54.7	&	58.1	&	2.3	&	1.6	&	493		&	...	\\
	3FGL J1742.6$-$3321$^\dagger$	&	...				&	2FGL J1742.5$-$3323	&	48.2	&	67.1	&	24.4	&	2.5	&	1.8	&	411		&	...	\\
	3FGL J1844.3$-$0344$^\dagger$	&	PSR J1844$-$0346&	2FGL J1844.3$-$0343c&	44.8	&	37.0	&	70.9	&	1.9	&	0.8	&	468		&	...	\\
	3FGL J1101.9$-$6053				&	...				&	...					&	23.3	&	40.8	&	61.3	&	2.4	&	1.8	&	519		&	spp	\\
	3FGL J2038.4$+$4212				&	...				&	...					&	45.7	&	51.1	&	95.8	&	0.5	&	0.6	&	340		&	...	\\
	3FGL J1849.4$-$0057				&	...				&	2FGL J1849.3$-$0055	&	45.1	&	23.8	&	16.6	&	13.5&	2.0	&	674		&	snr	\\
	3FGL J1112.0$-$6135				&	...				&	...					&	55.7	&	84.6	&	35.8	&	1.7	&	1.7	&	293		&	...	\\
	3FGL J1754.0$-$2538				&	...				&	2FGL J1754.4$-$2538c&	66.9	&	72.4	&	107.3	&	4.0	&	1.0	&	500		&	...	\\
	3FGL J0854.8$-$4503$^\dagger$	&	...				&	2FGL J0854.7$-$4501	&	44.9	&	47.5	&	54.9	&	5.0	&	1.7	&	737		&	...	\\
	3FGL J1857.2$+$0059				&	...				&	2FGL J1857.2$+$0055c&	57.1	&	32.6	&	113.2	&	4.5	&	1.3	&	383		&	...	\\
	3FGL J1740.5$-$2843				&	...				&	...					&	46.4	&	25.6	&	24.2	&	3.6	&	2.2	&	700		&	...	\\
	3FGL J1744.1$-$7619$^\dagger$	&	PSR J1744$-$7619&	2FGL J1744.1$-$7620	&	51.7	&	112.5	&	169.2	&	2.1	&	1.2	&	1759	&	...	\\
	3FGL J1035.7$-$6720$^\dagger$	&	PSR J1035$-$6720&	2FGL J1036.1$-$6722	&	47.0	&	80.6	&	120.2	&	2.3	&	1.4	&	1336	&	...	\\
	3FGL J1843.7$-$0322				&	...				&	...					&	70.6	&	65.5	&	54.5	&	3.7	&	2.6	&	1113	&	...	\\
	3FGL J0359.5$+$5413$^\dagger$	&	PSR J0359$+$5414&	2FGL J0359.5$+$5410	&	33.6	&	42.2	&	84.1	&	2.6	&	1.6	&	800		&	...	\\
	3FGL J1624.2$-$4041$^\dagger$	&	PSR J1624$-$4041&	2FGL J1624.1$-$4040	&	50.8	&	58.8	&	74.2	&	2.8	&	1.6	&	945		&	...	\\
	3FGL J1740.5$-$2726$^\dagger$	&	...				&	2FGL J1739.6$-$2726	&	43.2	&	39.9	&	31.1	&	1.8	&	2.0	&	401		&	...	\\
	3FGL J1827.3$-$1446				&	PSR J1827$-$1446&	2FGL J1827.4$-$1445c&	40.0	&	18.2	&	83.5	&	2.5	&	1.4	&	483		&	...	\\
	3FGL J2032.5$+$3921				&	...				&	...					&	49.4	&	46.2	&	34.1	&	0.4	&	0.8	&	233		&	...	\\
	3FGL J1638.6$-$4654				&	...				&	...					&	77.6	&	48.0	&	46.8	&	3.7	&	1.8	&	614		&	spp	\\
	3FGL J1925.4$+$1727				&	...				&	2FGL J1924.8$+$1724c&	47.3	&	42.2	&	22.3	&	1.2	&	1.2	&	157		&	...	\\
	3FGL J1857.9$+$0355				&	...				&	2FGL J1857.8$+$0355c&	55.6	&	31.5	&	29.6	&	1.6	&	1.1	&	146		&	...	\\
	3FGL J1208.4$-$6239$^\dagger$	&	...				&	2FGL J1208.5$-$6240	&	64.4	&	39.2	&	52.0	&	4.9	&	1.8	&	874		&	...	\\
	3FGL J1350.4$-$6224$^\dagger$	&	PSR J1350$-$6225&	2FGL J1349.9$-$6222	&	58.2	&	41.3	&	90.8	&	2.4	&	0.7	&	357		&	...	\\
	3FGL J1037.9$-$5843*			&	...				&	...					&	38.9	&	24.9	&	163.9	&	0.4	&	0.0	&	391		&	...	\\
	3FGL J2112.5$-$3044$^\dagger$	&	...				&	2FGL J2112.5$-$3042	&	51.8	&	69.0	&	151.0	&	2.8	&	1.1	&	1805	&	...	\\
	3FGL J1636.2$-$4709c			&	...				&	2FGL J1635.4$-$4717c&	57.4	&	13.7	&	4.4		&	11.5&	2.3	&	541		&	spp	\\
	3FGL J1358.5$-$6025				&	...				&	2FGL J1358.8$-$6027c&	53.2	&	32.8	&	21.1	&	5.7	&	2.2	&	639		&	...	\\
	3FGL J1048.2$-$5928				&	...				&	...					&	65.8	&	101.1	&	60.4	&	1.5	&	1.4	&	381		&	...	\\
	3FGL J2034.6$+$4302				&	...				&	...					&	41.4	&	50.7	&	112.6	&	0.4	&	0.3	&	324		&	...	\\
	3FGL J1754.0$-$2930$^\dagger$	&	...				&	2FGL J1754.1$-$2930	&	59.7	&	49.8	&	38.4	&	2.2	&	2.0	&	498		&	...	\\
	3FGL J1214.0$-$6236$^\dagger$	&	...				&	2FGL J1214.0$-$6237	&	58.0	&	20.3	&	15.7	&	13.1&	2.2	&	789		&	spp	\\
	3FGL J1652.8$-$4351				&	...				&	2FGL J1652.5$-$4351c&	64.6	&	31.0	&	62.0	&	1.3	&	0.9	&	184		&	...	\\
	3FGL J1317.6$-$6315				&	...				&	...					&	50.5	&	25.0	&	37.0	&	2.7	&	1.7	&	347		&	...	\\
	3FGL J2039.4$+$4111				&	...				&	2FGL J2040.1$+$4105c&	45.4	&	48.2	&	98.1	&	0.3	&	0.3	&	249		&	...	\\
	3FGL J1852.8$+$0158$^\dagger$*	&	...				&	2FGL J1852.8$+$0156c&	54.5	&	12.1	&	0.2		&	992.8&	2.8	&	838		&	...	\\
	3FGL J0631.6$+$0644				&	PSR J0631$+$0646&	2FGL J0631.6$+$0640	&	43.0	&	26.6	&	37.2	&	4.6	&	1.6	&	676		&	spp	\\
	3FGL J1840.1$-$0412*			&	...				&	2FGL J1840.3$-$0413c&	30.1	&	15.9	&	0.0		&	270.5&	2.5	&	416		&	spp	\\
	3FGL J1928.9$+$1739				&	...				&	2FGL J1928.8$+$1740c&	47.9	&	26.9	&	12.0	&	3.6	&	2.1	&	235		&	...	\\
	3FGL J0225.8$+$6159				&	...				&	2FGL J0225.9$+$6154c&	46.7	&	28.8	&	29.7	&	2.2	&	1.7	&	473		&	...	\\
	3FGL J0002.6$+$6218$^\dagger$	&	PSR J0002$+$6216&	2FGL J0002.7$+$6220	&	48.0	&	58.0	&	80.3	&	1.8	&	1.5	&	716		&	...	\\
	3FGL J1740.5$-$2642				&	...				&	...					&	33.4	&	23.2	&	34.1	&	2.5	&	1.8	&	222		&	...	\\
	3FGL J1834.5$-$0841$^\dagger$*	&	...				&	2FGL J1834.3$-$0848	&	57.1	&	0.5		&	0.1		&	216.7&	2.2	&	287		&	snr	\\
	3FGL J2042.4$+$4209				&	...				&	...					&	49.9	&	27.1	&	27.4	&	0.5	&	1.0	&	185		&	...	\\
	3FGL J1814.1$-$1734c$^\dagger$	&	...				&	2FGL J1814.1$-$1735c&	56.9	&	8.8		&	7.4		&	4.7	&	2.3	&	662		&	...	\\
	3FGL J2041.1$+$4736$^\dagger$	&	...				&	2FGL J2041.2$+$4735	&	56.3	&	38.0	&	15.9	&	10.3&	2.3	&	967		&	...	\\
	3FGL J1047.3$-$6005				&	...				&	2FGL J1046.8$-$6005c&	49.0	&	22.3	&	16.4	&	3.0	&	1.5	&	115		&	...	\\
	3FGL J2039.6$-$5618$^\dagger$	&	...				&	2FGL J2039.8$-$5620	&	34.6	&	30.4	&	60.3	&	3.9	&	1.6	&	1266	&	...	\\
	3FGL J1900.8$+$0337				&	...				&	...					&	45.9	&	44.9	&	4.7		&	10.4&	2.3	&	186		&	...	\\
	3FGL J0855.4$-$4818				&	...				&	...					&	33.8	&	53.0	&	66.4	&	0.5	&	0.9	&	288		&	...	\\
	3FGL J1747.7$-$2904				&	...				&	...					&	65.3	&	10.3	&	124.7	&	7.1	&	2.2	&	666		&	...	\\
	3FGL J0541.1$+$3553$^\dagger$	&	...				&	2FGL J0540.3$+$3549c&	35.2	&	37.3	&	33.0	&	1.8	&	1.9	&	329		&	...	\\
	3FGL J1549.1$-$5347c*			&	...				&	...					&	51.6	&	10.9	&	0.1		&	998.9&	2.9	&	1172	&	spp	\\
	3FGL J1039.1$-$5809				&	...				&	...					&	37.5	&	24.7	&	23.4	&	1.7	&	1.3	&	107		&	...	\\
	3FGL J1831.7$-$0230				&	...				&	...					&	31.1	&	17.8	&	2.1		&	17.4&	2.7	&	421		&	...	\\
	3FGL J1702.8$-$5656$^\dagger$	&	...				&	2FGL J1702.5$-$5654	&	58.8	&	46.9	&	53.1	&	3.4	&	2.1	&	1917	&	...	\\
	3FGL J1736.0$-$2701*			&	...				&	...					&	38.5	&	25.2	&	23.7	&	0.3	&	0.0	&	80		&	...	\\
	3FGL J2023.5$+$4126*			&	...				&	...					&	49.0	&	78.1	&	36.7	&	0.4	&	0.0	&	93		&	...	\\
	3FGL J1758.8$-$2346				&	...				&	...					&	41.8	&	11.8	&	5.4		&	20.8&	1.9	&	218		&	...	\\
	3FGL J2004.4$+$3338*			&	...				&	2FGL J2004.4$+$3339c&	50.3	&	13.5	&	0.0		&	866.5&	2.4	&	708		&	...	\\
	3FGL J0212.1$+$5320$^\dagger$	&	...				&	2FGL J0212.1$+$5318	&	51.5	&	45.9	&	82.0	&	3.3	&	1.5	&	1442	&	...	\\
	3FGL J1901.1$+$0728				&	...				&	...					&	55.3	&	25.8	&	10.5	&	6.6	&	2.0	&	134		&	...	\\
	3FGL J1503.5$-$5801				&	...				&	2FGL J1503.9$-$5800c&	67.5	&	26.3	&	18.7	&	3.7	&	2.0	&	359		&	...	\\
	3FGL J1850.5$-$0024				&	...				&	2FGL J1850.7$-$0014c&	64.3	&	14.6	&	2.8		&	7.7	&	2.3	&	216		&	...	\\
	3FGL J0933.9$-$6232$^\dagger$	&	...				&	2FGL J0934.0$-$6231	&	59.2	&	88.0	&	125.9	&	2.0	&	0.8	&	907		&	...	\\
	3FGL J1620.0$-$5101				&	...				&	...					&	50.5	&	9.7		&	1.0		&	64.9&	2.1	&	121		&	...	\\
	3FGL J1726.6$-$3530c			&	...				&	...					&	60.3	&	11.0	&	1.8		&	20.2&	2.6	&	335		&	...	\\
	3FGL J1919.9$+$1407				&	...				&	...					&	67.7	&	17.6	&	0.3		&	87.2&	2.7	&	642		&	...	\\
	3FGL J1119.9$-$2204$^\dagger$	&	...				&	2FGL J1120.0$-$2204	&	62.6	&	103.2	&	156.9	&	1.7	&	1.3	&	1949	&	...	\\
	3FGL J0907.0$-$4802*			&	...				&	...					&	40.8	&	29.3	&	28.0	&	0.4	&	0.2	&	123		&	...	\\
	3FGL J1718.0$-$3726				&	...				&	2FGL J1718.1$-$3725	&	41.6	&	1.5		&	2.0		&	80.1&	2.1	&	593		&	snr	\\
	3FGL J1859.6$+$0102				&	...				&	...					&	68.6	&	18.9	&	13.1	&	3.5	&	1.8	&	150		&	...	\\
	3FGL J2035.0$+$3634				&	...				&	2FGL J2034.9$+$3632	&	52.6	&	39.2	&	57.5	&	2.8	&	0.8	&	401		&	...	\\
	3FGL J1345.1$-$6224				&	...				&	...					&	58.3	&	12.8	&	1.3		&	29.5&	2.7	&	568		&	spp	\\
	3FGL J0744.1$-$2523$^\dagger$	&	...				&	2FGL J0744.1$-$2523	&	61.3	&	40.9	&	55.3	&	3.2	&	1.8	&	666		&	...	\\
	3FGL J0426.7$+$5437$^\dagger$	&	...				&	2FGL J0426.7$+$5434	&	51.8	&	63.9	&	59.0	&	1.7	&	2.1	&	1235	&	...	\\
	3FGL J1539.2$-$3324$^\dagger$	&	...				&	2FGL J1539.2$-$3325	&	57.9	&	102.9	&	129.3	&	2.3	&	0.4	&	694		&	...	\\
	3FGL J1641.1$-$4619c*			&	...				&	...					&	39.4	&	1.0		&	0.2		&	150.0&	2.3	&	292		&	spp	\\
	3FGL J1528.3$-$5836				&	PSR J1528$-$5838&	2FGL J1528.0$-$5841	&	68.7	&	44.9	&	41.4	&	4.0	&	1.6	&	452		&	...	\\
	3FGL J1857.8$+$0129c			&	...				&	2FGL J1858.5$+$0129c&	41.5	&	11.2	&	32.2	&	2.2	&	1.4	&	131		&	...	\\
	3FGL J1855.4$+$0454				&	...				&	...					&	38.6	&	6.6		&	4.4		&	10.5&	2.4	&	193		&	...	\\
	3FGL J1650.0$-$4438c*			&	...				&	...					&	58.8	&	1.0		&	0.1		&	918.9&	3.1	&	843		&	...	\\
	3FGL J0901.6$-$4700$^\dagger$	&	...				&	2FGL J0901.7$-$4655	&	55.1	&	30.0	&	52.7	&	1.0	&	1.2	&	221		&	...	\\
	3FGL J1329.8$-$6109				&	...				&	2FGL J1329.7$-$6108	&	55.7	&	22.5	&	21.1	&	4.9	&	1.6	&	246		&	...	\\
	3FGL J1639.4$-$5146				&	...				&	2FGL J1639.8$-$5145	&	58.0	&	4.2		&	2.8		&	46.3&	2.3	&	945		&	...	\\
	3FGL J1833.9$-$0711*			&	...				&	...					&	82.1	&	1.6		&	0.4		&	997.5&	2.3	&	482		&	spp	\\
	3FGL J1814.0$-$1757c			&	...				&	...					&	50.1	&	7.1		&	5.3		&	3.9	&	1.4	&	83		&	...	\\
	3FGL J1139.0$-$6244				&	...				&	2FGL J1138.8$-$6233c&	29.5	&	7.5		&	16.5	&	8.6	&	1.9	&	278		&	...	\\
	3FGL J1626.2$-$2428c			&	...				&	...					&	46.9	&	15.9	&	7.8		&	7.8	&	2.1	&	392		&	...	\\
	3FGL J1212.2$-$6251				&	...				&	...					&	53.7	&	1.4		&	12.9	&	45.8&	2.4	&	426		&	spp	\\
	\tablecomments{The source list sorted with the logarithmic likelihood from GMM. Sources with $\dagger$ were searched in previous Einstein@Home/Altas blind search survey. Sources with ``*'' means the spectral fit result in abnormal value. Columns 2 and 3 list the name of the pulsar detected in this survey and the assoicated 2FGL name. Columns 4 and 5 list the varibility index and cuvature TS listed in the 3FGL catalog. Columns 6-9 are the spectral parameters result from the binned likelihood analysis with Pointlike. Column 10 is the source assiocation flag taken from the 3FGL catalog, ``pwn'' and ``snr'' represent possible assiocation with pulsar wind nebula (PWN) and supernova remnant (SNR) respectivity, sources with class ``spp'' are special case indicates potential assoication with SNR or PWN.}
	\enddata
\end{deluxetable*}


==> sens_table.tex <==
\begin{deluxetable*}{cccccccc}
  \tablecaption{\label{t:minimum_pulsed_fraction} Pulsed fraction upper limits}
  \tablecolumns{8}
  \tablehead{
    \colhead{3FGL Name} & \colhead{$p_{\rm s}^\ast$\tablenotemark{a}} & \colhead{$p_{\rm s}$\tablenotemark{b}} & \colhead{$N_{\rm FFT}$\tablenotemark{c}$/ 10^6$} & \colhead{3FGL Name} & \colhead{$p_{\rm s}^\ast$\tablenotemark{a}} & \colhead{$p_{\rm s}$\tablenotemark{b}} & \colhead{$N_{\rm FFT}$\tablenotemark{c}$/ 10^6$}
  }
  \startdata
    \textbf{J0002.6$+$6218} & $\mathbf{0.68}$ & $\mathbf{0.96}$ & $\mathbf{38.78}$ \phs& J1726.6$-$3530 & $> 1$ & \nodata & $292.96$ \\
    J0212.1$+$5320 & $0.56$  & \nodata & $73.31$ \phs&J1736.0$-$2701 & $> 1$ & \nodata & $160.02$ \\
    J0223.6$+$6204 & $0.53$  & \nodata & $304.66$ \phs&J1740.5$-$2642 & $> 1$ & \nodata & $56.71$ \\
    J0225.8$+$6159 & $0.79$  & \nodata & $400.20$ \phs&J1740.5$-$2726 & $0.86$ & \nodata & $177.86$ \\
    \textbf{J0359.5$+$5413} & $\mathbf{0.64}$ & $\mathbf{0.87}$ & $\mathbf{258.10}$ \phs& J1740.5$-$2843 & $0.71$ & \nodata & $117.70$ \\
    J0426.7$+$5437 & $0.50$  & \nodata & $45.44$ \phs&J1742.6$-$3321 & $0.83$ & \nodata & $231.76$ \\
    J0541.1$+$3553 & $0.90$  & \nodata & $776.03$ \phs&\textbf{J1744.1$-$7619\tablenotemark{d}} & $\mathbf{0.54}$ & $\mathbf{0.72}$ & $\mathbf{275.49}$ \\
    \textbf{J0631.6$+$0644} & $\mathbf{0.74}$ & $\mathbf{0.90}$ & $\mathbf{10.11}$ \phs& J1745.1$-$3011 & $0.77$ & \nodata & $165.41$ \\
    J0634.1$+$0424 & $0.46$  & \nodata & $1140.90$ \phs&J1745.3$-$2903 & $0.33$ & \nodata & $16.65$ \\
    J0744.1$-$2523 & $0.72$  & \nodata & $26.92$ \phs&J1746.3$-$2851 & $0.39$ & \nodata & $17.16$ \\
    J0854.8$-$4503 & $0.71$  & \nodata & $579.82$ \phs&J1747.0$-$2828 & $0.49$ & \nodata & $45.69$ \\
    J0855.4$-$4818 & $0.96$  & \nodata & $4899.56$ \phs&J1747.7$-$2904 & $0.81$ & \nodata & $43.13$ \\
    J0901.6$-$4700 & $> 1$  & \nodata & $415.84$ \phs&J1748.3$-$2815 & $0.78$ & \nodata & $23.44$ \\
    J0907.0$-$4802 & $> 1$  & \nodata & $860.15$ \phs&J1749.2$-$2911 & $> 1$ & \nodata & $193.65$ \\
    J0933.9$-$6232 & $0.74$  & \nodata & $133.98$ \phs&J1754.0$-$2538 & $0.81$ & \nodata & $11.29$ \\
    J1026.2$-$5730 & $0.79$  & \nodata & $713.27$ \phs&J1754.0$-$2930 & $0.77$ & \nodata & $79.32$ \\
    \textbf{J1035.7$-$6720\tablenotemark{d}} & $\mathbf{0.56}$ & $\mathbf{0.93}$ & $\mathbf{353.57}$ \phs& J1758.8$-$2346 & $> 1$ & \nodata & $21.08$ \\
    J1037.9$-$5843 & $0.83$  & \nodata & $748.28$ \phs&J1800.8$-$2402 & $0.75$ & \nodata & $12.44$ \\
    J1039.1$-$5809 & $> 1$  & \nodata & $7498.83$ \phs&J1814.0$-$1757 & $> 1$ & \nodata & $33.23$ \\
    J1047.3$-$6005 & $> 1$  & \nodata & $1607.52$ \phs&J1814.1$-$1734 & $0.80$ & \nodata & $43.69$ \\
    J1048.2$-$5928 & $0.88$  & \nodata & $651.27$ \phs&J1823.2$-$1339 & $0.58$ & \nodata & $41.60$ \\
    \textbf{J1056.7$-$5853} & $\mathbf{0.70}$ & $\mathbf{0.68}$ & $\mathbf{1793.05}$ \phs& \textbf{J1827.3$-$1446} & $\mathbf{0.78}$ & $\mathbf{1.00}$ & $\mathbf{169.81}$ \\
    J1101.9$-$6053 & $0.77$  & \nodata & $1676.99$ \phs&J1831.7$-$0230 & $0.91$ & \nodata & $624.00$ \\
    \textbf{J1104.9$-$6036} & $\mathbf{0.66}$ & $\mathbf{0.71}$ & $\mathbf{499.71}$ \phs& J1833.9$-$0711 & $0.88$ & \nodata & $27.47$ \\
    J1111.9$-$6038 & $0.35$  & \nodata & $113.63$ \phs&J1834.5$-$0841 & $> 1$ & \nodata & $208.28$ \\
    J1112.0$-$6135 & $0.98$  & \nodata & $2341.02$ \phs&J1839.3$-$0552 & $0.63$ & \nodata & $104.52$ \\
    J1119.9$-$2204 & $0.51$  & \nodata & $13.72$ \phs&J1840.1$-$0412 & $0.97$ & \nodata & $145.45$ \\
    J1139.0$-$6244 & $> 1$  & \nodata & $42.51$ \phs&J1843.7$-$0322 & $0.68$ & \nodata & $747.26$ \\
    \textbf{J1208.4$-$6239\tablenotemark{d}} & $\mathbf{0.63}$ & $\mathbf{0.53}$ & $\mathbf{92.51}$ \phs& \textbf{J1844.3$-$0344} & $\mathbf{0.78}$ & $\mathbf{0.88}$ & $\mathbf{318.79}$ \\
    J1212.2$-$6251 & $0.90$  & \nodata & $61.67$ \phs&J1848.4$-$0141 & $0.58$ & \nodata & $727.88$ \\
    J1214.0$-$6236 & $0.66$  & \nodata & $146.94$ \phs&J1849.4$-$0057 & $0.71$ & \nodata & $176.94$ \\
    J1306.4$-$6043 & $0.61$  & \nodata & $161.88$ \phs&J1850.5$-$0024 & $> 1$ & \nodata & $458.08$ \\
    J1317.6$-$6315 & $0.92$  & \nodata & $314.90$ \phs&J1852.8$+$0158 & $0.78$ & \nodata & $379.46$ \\
    J1329.8$-$6109 & $> 1$  & \nodata & $42.10$ \phs&J1855.4$+$0454 & $> 1$ & \nodata & $95.62$ \\
    J1345.1$-$6224 & $0.87$  & \nodata & $182.65$ \phs&J1857.2$+$0059 & $0.90$ & \nodata & $220.81$ \\
    \textbf{J1350.4$-$6224} & $\mathbf{0.95}$ & $\mathbf{1.00}$ & $\mathbf{100.80}$ \phs& J1857.8$+$0129 & $> 1$ & \nodata & $109.05$ \\
    J1358.5$-$6025 & $0.71$  & \nodata & $199.81$ \phs&J1857.9$+$0210 & $0.73$ & \nodata & $459.00$ \\
    J1405.4$-$6119 & $0.48$  & \nodata & $198.20$ \phs&J1857.9$+$0355 & $> 1$ & \nodata & $270.39$ \\
    J1503.5$-$5801 & $0.92$  & \nodata & $459.50$ \phs&J1859.6$+$0102 & $> 1$ & \nodata & $120.74$ \\
    \textbf{J1528.3$-$5836} & $\mathbf{0.88}$ & $\mathbf{0.98}$ & $\mathbf{21.22}$ \phs& J1900.8$+$0337 & $> 1$ & \nodata & $354.12$ \\
    J1539.2$-$3324 & $0.86$  & \nodata & $7.42$ \phs&J1901.1$+$0728 & $> 1$ & \nodata & $278.80$ \\
    J1549.1$-$5347 & $0.69$  & \nodata & $663.95$ \phs&\textbf{J1906.6$+$0720} & $\mathbf{0.47}$ & $\mathbf{0.77}$ & $\mathbf{206.02}$ \\
    J1552.8$-$5330 & $> 1$  & \nodata & $930.32$ \phs&J1910.9$+$0906 & $0.31$ & \nodata & $47.32$ \\
    J1620.0$-$5101 & $> 1$  & \nodata & $384.50$ \phs&J1919.9$+$1407 & $0.83$ & \nodata & $383.20$ \\
    \textbf{J1622.9$-$5004} & $\mathbf{0.62}$ & $\mathbf{0.74}$ & $\mathbf{78.62}$ \phs& J1925.4$+$1727 & $> 1$ & \nodata & $1704.54$ \\
    \textbf{J1624.2$-$4041} & $\mathbf{0.61}$ & $\mathbf{0.68}$ & $\mathbf{192.42}$ \phs& J1928.9$+$1739 & $> 1$ & \nodata & $2680.58$ \\
    J1625.1$-$0021 & $0.57$  & \nodata & $154.54$ \phs&J2004.4$+$3338 & $0.70$ & \nodata & $84.87$ \\
    J1626.2$-$2428 & $0.87$  & \nodata & $10.64$ \phs&\textbf{J2017.9$+$3627} & $\mathbf{0.43}$ & $\mathbf{0.64}$ & $\mathbf{178.21}$ \\
    J1636.2$-$4709 & $0.89$  & \nodata & $405.59$ \phs&J2023.5$+$4126 & $> 1$ & \nodata & $776.94$ \\
    J1636.2$-$4734 & $0.54$  & \nodata & $321.30$ \phs&J2032.5$+$3921 & $> 1$ & \nodata & $541.70$ \\
    J1638.6$-$4654 & $0.73$  & \nodata & $102.88$ \phs&J2034.6$+$4302 & $0.90$ & \nodata & $1601.98$ \\
    J1639.4$-$5146 & $0.63$  & \nodata & $9.24$ \phs&J2035.0$+$3634 & $1.00$ & \nodata & $26.52$ \\
    J1641.1$-$4619 & $> 1$  & \nodata & $14.19$ \phs&J2038.4$+$4212 & $0.87$ & \nodata & $845.17$ \\
    J1650.0$-$4438 & $0.87$  & \nodata & $161.85$ \phs&J2039.4$+$4111 & $> 1$ & \nodata & $525.98$ \\
    \textbf{J1650.3$-$4600} & $\mathbf{0.60}$ & $\mathbf{0.78}$ & $\mathbf{139.09}$ \phs& J2039.6$-$5618 & $0.61$ & \nodata & $91.84$ \\
    J1652.8$-$4351 & $> 1$  & \nodata & $741.14$ \phs&J2041.1$+$4736 & $0.58$ & \nodata & $170.62$ \\
    J1702.8$-$5656 & $0.43$  & \nodata & $96.18$ \phs&J2042.4$+$4209 & $> 1$ & \nodata & $5359.83$ \\
    J1714.5$-$3832 & $0.39$  & \nodata & $67.93$ \phs&J2112.5$-$3044 & $0.56$ & \nodata & $22.79$ \\
    J1718.0$-$3726 & $0.79$  & \nodata & $2.56$ \phs&J2323.4$+$5849 & $0.47$ & \nodata & $63.63$ \\
  \enddata
  \tablecomments{Sources in which pulsars were discovered by the \EAH{} survey are shown in bold.}  \tablenotetext{a}{Estimated values for the pulsed fraction above which we expect to detect a signal from each source with 95\% probability.}  \tablenotetext{b}{Measured pulse fraction for newly discovered pulsars.}  \tablenotetext{c}{Number of FFTs required to search the entire parameter space for each source.}  \tablenotetext{d}{These pulsars have timing properties warranting further individual investigation, and will be presented in later works.}
\end{deluxetable*}


==> source_list.tex.20170314 <==
\clearpage 

\LongTables

\begin{deluxetable*}{lcccrrrrrrcc}[p]		
	
	\tablecaption{\label{t:source_list} Ranked source list}
	\tablecolumns{10}
	\tablehead{
		\colhead{3FGL Name}&
		\colhead{Searched R.A.}&
		\colhead{Searched Decl.}&
		\colhead{Search Radius}&
		\colhead{VI}&		
		\colhead{$\textrm{TS}_\textrm{curve}$}&
		\colhead{$\textrm{TS}_\textrm{cut}$}&
		\colhead{$E_\textrm{cut}$}&
		\colhead{$\Gamma$}&
		\colhead{TS}&
		\colhead{log $R_{S}$}&
		\colhead{Class}\\
		\colhead{}&
		\colhead{(J2000)}&
		\colhead{(J2000)}&
		\colhead{(arcmin)}&
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{(GeV)}&
		\colhead{}&
		\colhead{}&
		\colhead{}&
		\colhead{}
	}
	

3FGL J1745.3$-$2903c	&	17:45:22.32	&	$-$29:03:46.80	&	1.37	&	48.42	&	275.2	&	378.7	&	2.2	&	1.4	&	3407	&	18.85	&	...	\\
3FGL J1746.3$-$2851c	&	17:46:22.51	&	$-$28:51:45.72	&	1.42	&	57.06	&	113	&	364.69	&	4.0	&	1.5	&	2373	&	14.31	&	pwn	\\
\textbf{3FGL J2017.9$+$3627}	&	20:17:56.33	&	$+$36:27:32.76	&	2.06	&	39.86	&	179.27	&	198.86	&	1.9	&	1.4	&	1876	&	13.61	&	...	\\
3FGL J1839.3$-$0552	&	18:39:23.52	&	$-$05:52:53.76	&	2.05	&	37.43	&	83.71	&	135.1	&	2.3	&	1.2	&	714	&	13.26	&	...	\\
\textbf{3FGL J1906.6$+$0720}$^\dagger$	&	19:06:41.14	&	$+$07:20:02.04	&	2.22	&	41.7	&	87.9	&	68.6	&	7.0	&	2.0	&	1580	&	12.51	&	...	\\
3FGL J1910.9$+$0906$^\dagger$	&	19:10:58.61	&	$+$09:06:01.80	&	1.03	&	52.13	&	53.18	&	17.41	&	41.7	&	2.1	&	4790	&	12.31	&	snr	\\
3FGL J1636.2$-$4734	&	16:36:16.49	&	$-$47:34:49.08	&	3.05	&	54.63	&	105.95	&	47.14	&	7.1	&	1.9	&	1180	&	12.28	&	snr	\\
3FGL J1848.4$-$0141	&	18:48:28.39	&	$-$01:41:33.72	&	4.85	&	52.63	&	109.04	&	13.79	&	9.8	&	2.5	&	1457	&	11.81	&	...	\\
3FGL J1405.4$-$6119$^\dagger$	&	14:05:25.46	&	$-$61:19:00.48	&	1.88	&	43.93	&	61.08	&	19.69	&	8.2	&	2.1	&	1671	&	11.39	&	...	\\
3FGL J1111.9$-$6038$^\dagger$	&	11:11:58.44	&	$-$60:38:27.96	&	1.31	&	46.69	&	81.4	&	58.48	&	10.4	&	1.9	&	3624	&	11.36	&	spp	\\
3FGL J1748.3$-$2815c	&	17:48:22.20	&	$-$28:15:32.04	&	1.82	&	34.06	&	77.37	&	68.59	&	4.7	&	1.4	&	489	&	11.26	&	...	\\
\textbf{3FGL J1622.9$-$5004}$^\dagger$	&	16:22:54.31	&	$-$50:04:31.08	&	1.45	&	54.35	&	72.44	&	73.27	&	8.0	&	1.6	&	891	&	10.21	&	...	\\
3FGL J0223.6$+$6204$^\dagger$	&	02:23:37.46	&	$+$62:04:51.96	&	2.34	&	41.77	&	86.32	&	182.58	&	1.8	&	1.5	&	1089	&	9.78	&	...	\\
3FGL J1823.2$-$1339$^\dagger$	&	18:23:16.90	&	$-$13:39:04.68	&	1.73	&	47.54	&	29.72	&	47.36	&	9.0	&	1.9	&	1004	&	9.72	&	...	\\
3FGL J1745.1$-$3011	&	17:45:11.30	&	$-$30:11:57.84	&	4.11	&	59.68	&	92.72	&	88.83	&	0.6	&	0.4	&	459	&	9.69	&	spp	\\
3FGL J1800.8$-$2402$^\dagger$	&	18:00:53.18	&	$-$24:02:06.36	&	2.09	&	46.65	&	36.4	&	21.3	&	11.3	&	1.7	&	575	&	9.69	&	...	\\
3FGL J1749.2$-$2911	&	17:49:15.58	&	$-$29:11:34.44	&	4.81	&	41.77	&	50.89	&	43.64	&	1.6	&	1.3	&	265	&	9.62	&	...	\\
3FGL J1306.4$-$6043$^\dagger$	&	13:06:27.50	&	$-$60:43:54.12	&	1.65	&	35.69	&	65.89	&	42.63	&	8.6	&	1.7	&	1108	&	9.59	&	...	\\
\textbf{3FGL J1104.9$-$6036}$^\dagger$	&	11:04:59.42	&	$-$60:36:32.76	&	2.73	&	43.09	&	77.36	&	64.59	&	3.6	&	1.7	&	769	&	9.42	&	...	\\
3FGL J0634.1$+$0424	&	06:34:06.79	&	$+$04:24:22.32	&	6.52	&	42.87	&	123.32	&	60.17	&	1.8	&	2.2	&	1421	&	9.41	&	...	\\
3FGL J1552.8$-$5330	&	15:52:50.90	&	$-$53:30:47.16	&	4.65	&	46.44	&	56.59	&	50.32	&	1.8	&	1.0	&	210	&	9.26	&	...	\\
3FGL J1747.0$-$2828	&	17:47:05.98	&	$-$28:28:54.84	&	2.44	&	90.61	&	159.71	&	135.26	&	2.5	&	1.8	&	1676	&	9.22	&	...	\\
\textbf{3FGL J1650.3$-$4600}	&	16:50:23.76	&	$-$46:00:50.76	&	2.09	&	55.06	&	54.61	&	54.97	&	4.8	&	1.8	&	897	&	9.19	&	...	\\
3FGL J2323.4$+$5849	&	23:23:28.85	&	$+$58:49:09.48	&	1.00	&	40.07	&	62.43	&	39.06	&	26.4	&	1.6	&	2568	&	9.17	&	snr	\\
3FGL J1625.1$-$0021$^\dagger$	&	16:25:07.06	&	$-$00:21:30.96	&	2.25	&	37.31	&	104.31	&	201.42	&	1.9	&	0.8	&	1778	&	8.98	&	...	\\
3FGL J1714.5$-$3832	&	17:14:34.27	&	$-$38:32:55.68	&	1.76	&	68.77	&	39.31	&	23.25	&	14.7	&	2.2	&	2649	&	8.95	&	snr	\\
3FGL J1857.9$+$0210$^\dagger$	&	18:57:57.65	&	$+$02:10:13.44	&	3.61	&	50.62	&	42.8	&	50.49	&	3.2	&	1.9	&	601	&	8.89	&	...	\\
\textbf{3FGL J1056.7$-$5853}$^\dagger$	&	10:56:42.86	&	$-$58:53:45.60	&	5.18	&	35.71	&	88.18	&	126.08	&	1.1	&	1.5	&	596	&	8.83	&	...	\\
3FGL J1026.2$-$5730	&	10:26:14.33	&	$-$57:30:59.76	&	3.23	&	50.42	&	54.72	&	58.12	&	2.3	&	1.6	&	493	&	8.26	&	...	\\
3FGL J1742.6$-$3321$^\dagger$	&	17:42:39.60	&	$-$33:21:22.32	&	4.00	&	48.24	&	67.12	&	24.42	&	2.5	&	1.8	&	411	&	8.20	&	...	\\
\textbf{3FGL J1844.3$-$0344}$^\dagger$	&	18:44:23.93	&	$-$03:44:48.48	&	3.39	&	44.78	&	37.01	&	70.92	&	1.9	&	0.8	&	468	&	8.12	&	...	\\
3FGL J1101.9$-$6053	&	11:01:55.46	&	$-$60:53:45.96	&	4.99	&	23.32	&	40.83	&	61.28	&	2.4	&	1.8	&	519	&	7.95	&	spp	\\
3FGL J2038.4$+$4212	&	20:38:29.95	&	$+$42:12:30.60	&	3.53	&	45.67	&	51.06	&	95.81	&	0.5	&	0.6	&	340	&	7.92	&	...	\\
3FGL J1849.4$-$0057	&	18:49:25.30	&	$-$00:57:06.48	&	2.36	&	45.11	&	23.82	&	16.55	&	13.5	&	2.0	&	674	&	7.86	&	snr	\\
3FGL J1112.0$-$6135	&	11:12:04.03	&	$-$61:35:03.12	&	5.92	&	55.72	&	84.61	&	35.82	&	1.7	&	1.7	&	293	&	7.84	&	...	\\
3FGL J1754.0$-$2538	&	17:54:02.02	&	$-$25:38:54.96	&	1.75	&	66.89	&	72.39	&	107.28	&	4.0	&	1.0	&	500	&	7.73	&	...	\\
3FGL J0854.8$-$4503$^\dagger$	&	08:54:50.59	&	$-$45:03:41.76	&	2.91	&	44.94	&	47.48	&	54.92	&	5.0	&	1.7	&	737	&	7.68	&	...	\\
3FGL J1857.2$+$0059	&	18:57:14.28	&	$+$00:59:10.68	&	2.54	&	57.14	&	32.56	&	113.21	&	4.5	&	1.3	&	383	&	7.67	&	...	\\
3FGL J1740.5$-$2843	&	17:40:30.00	&	$-$28:43:01.20	&	3.91	&	46.42	&	25.6	&	24.21	&	3.6	&	2.2	&	700	&	7.66	&	...	\\
\textbf{3FGL J1744.1$-$7619}$^\dagger$	&	17:44:10.85	&	$-$76:19:42.96	&	2.08	&	51.73	&	112.45	&	169.22	&	2.1	&	1.2	&	1759	&	7.61	&	...	\\
\textbf{3FGL J1035.7$-$6720}$^\dagger$	&	10:35:42.24	&	$-$67:20:00.60	&	2.23	&	47.01	&	80.61	&	120.2	&	2.3	&	1.4	&	1336	&	7.39	&	...	\\
3FGL J1843.7$-$0322	&	18:43:42.77	&	$-$03:22:37.92	&	5.11	&	70.63	&	65.49	&	54.52	&	3.7	&	2.6	&	1113	&	7.37	&	...	\\
\textbf{3FGL J0359.5$+$5413}$^\dagger$	&	03:59:31.46	&	$+$54:13:19.20	&	2.44	&	33.63	&	42.17	&	84.06	&	2.6	&	1.6	&	800	&	7.19	&	...	\\
\textbf{3FGL J1624.2$-$4041}$^\dagger$	&	16:24:14.26	&	$-$40:41:11.40	&	2.68	&	50.8	&	58.82	&	74.16	&	2.8	&	1.6	&	945	&	7.18	&	...	\\
3FGL J1740.5$-$2726$^\dagger$	&	17:40:32.28	&	$-$27:27:00.00	&	5.53	&	43.15	&	39.91	&	31.07	&	1.8	&	2.0	&	401	&	7.04	&	...	\\
\textbf{3FGL J1827.3$-$1446}	&	18:27:20.16	&	$-$14:46:01.92	&	3.70	&	40	&	18.21	&	83.49	&	2.5	&	1.4	&	483	&	6.96	&	...	\\
\hline\\
3FGL J2032.5$+$3921	&	20:32:29.78	&	$+$39:25:20.60	&	1.23	&	49.41	&	46.16	&	34.1	&	0.4	&	0.8	&	233	&	6.95	&	...	\\
3FGL J1638.6$-$4654	&	16:38:40.16	&	$-$46:54:06.33	&	0.75	&	77.58	&	47.95	&	46.81	&	3.7	&	1.8	&	614	&	6.84	&	spp	\\
3FGL J1925.4$+$1727	&	19:24:58.98	&	$+$17:24:41.84	&	2.46	&	47.33	&	42.21	&	22.26	&	1.2	&	1.2	&	157	&	6.70	&	...	\\
3FGL J1857.9$+$0355	&	18:58:03.73	&	$+$03:55:08.04	&	1.15	&	55.58	&	31.47	&	29.64	&	1.6	&	1.1	&	146	&	6.55	&	...	\\
\textbf{3FGL J1208.4$-$6239}$^\dagger$	&	12:08:26.89	&	$-$62:39:26.13	&	0.52	&	64.44	&	39.22	&	51.98	&	4.9	&	1.8	&	874	&	6.43	&	...	\\
\textbf{3FGL J1350.4$-$6224}$^\dagger$	&	13:50:34.69	&	$-$62:23:43.53	&	0.57	&	58.24	&	41.33	&	90.78	&	2.4	&	0.7	&	357	&	6.41	&	...	\\
3FGL J1037.9$-$5843*	&	10:38:01.49	&	$-$58:44:20.62	&	1.43	&	38.88	&	24.86	&	163.93	&	0.4	&	0.0	&	391	&	6.32	&	...	\\
3FGL J2112.5$-$3044$^\dagger$	&	21:12:32.39	&	$-$30:43:58.53	&	0.46	&	51.84	&	69.04	&	150.97	&	2.8	&	1.1	&	1805	&	6.25	&	...	\\
3FGL J1636.2$-$4709c	&	16:36:22.32	&	$-$47:09:53.05	&	1.47	&	57.44	&	13.67	&	4.35	&	11.5	&	2.3	&	541	&	6.17	&	spp	\\
3FGL J1358.5$-$6025	&	13:58:24.20	&	$-$60:25:30.56	&	0.81	&	53.16	&	32.84	&	21.1	&	5.7	&	2.2	&	639	&	6.15	&	...	\\
3FGL J1048.2$-$5928	&	10:48:40.66	&	$-$59:26:03.43	&	1.33	&	65.78	&	101.07	&	60.41	&	1.5	&	1.4	&	381	&	6.11	&	...	\\
3FGL J2034.6$+$4302	&	20:34:58.42	&	$+$43:05:08.99	&	2.10	&	41.4	&	50.67	&	112.64	&	0.4	&	0.3	&	324	&	6.11	&	...	\\
3FGL J1754.0$-$2930$^\dagger$	&	17:54:14.33	&	$-$29:32:08.04	&	1.24	&	59.67	&	49.75	&	38.35	&	2.2	&	2.0	&	498	&	6.06	&	...	\\
3FGL J1214.0$-$6236$^\dagger$	&	12:14:10.04	&	$-$62:36:16.69	&	0.66	&	58.02	&	20.3	&	15.68	&	13.1	&	2.2	&	789	&	6.05	&	spp	\\
3FGL J1652.8$-$4351	&	16:52:32.63	&	$-$43:56:50.10	&	2.13	&	64.55	&	30.95	&	61.97	&	1.3	&	0.9	&	184	&	6.00	&	...	\\
3FGL J1317.6$-$6315	&	13:17:35.62	&	$-$63:17:18.00	&	0.99	&	50.53	&	24.95	&	36.99	&	2.7	&	1.7	&	347	&	5.99	&	...	\\
3FGL J2039.4$+$4111	&	20:39:45.84	&	$+$41:09:34.39	&	1.20	&	45.39	&	48.23	&	98.07	&	0.3	&	0.3	&	249	&	5.91	&	...	\\
3FGL J1852.8$+$0158$^\dagger$*	&	18:52:27.92	&	$+$02:01:37.54	&	1.39	&	54.52	&	12.05	&	0.17	&	992.8	&	2.8	&	838	&	5.89	&	...	\\
\textbf{3FGL J0631.6$+$0644}	&	06:31:49.76	&	$+$06:44:46.66	&	0.64	&	43.04	&	26.63	&	37.16	&	4.6	&	1.6	&	676	&	5.84	&	spp	\\
3FGL J1840.1$-$0412*	&	18:40:06.15	&	$-$04:11:35.22	&	0.98	&	30.14	&	15.92	&	0.02	&	270.5	&	2.5	&	416	&	5.83	&	spp	\\
3FGL J1928.9$+$1739	&	19:29:02.93	&	$+$17:34:58.90	&	3.05	&	47.86	&	26.89	&	12.02	&	3.6	&	2.1	&	235	&	5.79	&	...	\\
3FGL J0225.8$+$6159	&	02:26:20.37	&	$+$62:00:10.48	&	1.16	&	46.69	&	28.83	&	29.69	&	2.2	&	1.7	&	473	&	5.77	&	...	\\
\textbf{3FGL J0002.6$+$6218}$^\dagger$	&	00:02:48.88	&	$+$62:16:54.71	&	0.75	&	48.02	&	57.97	&	80.32	&	1.8	&	1.5	&	716	&	5.76	&	...	\\
3FGL J1740.5$-$2642	&	17:40:41.52	&	$-$26:39:52.98	&	1.43	&	33.42	&	23.23	&	34.12	&	2.5	&	1.8	&	222	&	5.74	&	...	\\
3FGL J1834.5$-$0841$^\dagger$*	&	18:34:31.66	&	$-$08:40:15.75	&	1.34	&	57.1	&	0.49	&	0.05	&	216.7	&	2.2	&	287	&	5.72	&	snr	\\
3FGL J2042.4$+$4209	&	20:42:39.77	&	$+$42:09:19.64	&	3.83	&	49.9	&	27.05	&	27.37	&	0.5	&	1.0	&	185	&	5.68	&	...	\\
3FGL J1814.0$-$1757c	&	18:13:24.52	&	$-$17:53:55.97	&	1.94	&	56.91	&	8.84	&	7.39	&	4.7	&	2.3	&	662	&	5.59	&	...	\\
3FGL J2041.1$+$4736$^\dagger$	&	20:41:08.34	&	$+$47:35:50.81	&	0.67	&	56.28	&	38.02	&	15.86	&	10.3	&	2.3	&	967	&	5.53	&	...	\\
3FGL J1047.3$-$6005	&	10:47:21.66	&	$-$60:05:11.01	&	2.07	&	49.04	&	22.32	&	16.4	&	3.0	&	1.5	&	115	&	5.52	&	...	\\
3FGL J2039.6$-$5618$^\dagger$	&	20:39:36.25	&	$-$56:17:12.94	&	0.61	&	34.6	&	30.38	&	60.25	&	3.9	&	1.6	&	1266	&	5.47	&	...	\\
3FGL J1900.8$+$0337	&	19:00:37.96	&	$+$03:39:10.57	&	1.31	&	45.87	&	44.91	&	4.66	&	10.4	&	2.3	&	186	&	5.42	&	...	\\
3FGL J0855.4$-$4818	&	08:55:18.44	&	$-$48:14:13.02	&	3.56	&	33.84	&	53	&	66.39	&	0.5	&	0.9	&	288	&	5.39	&	...	\\
3FGL J1747.7$-$2904	&	17:47:51.94	&	$-$29:01:49.54	&	0.98	&	65.34	&	10.32	&	124.73	&	7.1	&	2.2	&	666	&	5.37	&	...	\\
3FGL J0541.1$+$3553$^\dagger$	&	05:40:47.47	&	$+$35:54:40.72	&	2.84	&	35.17	&	37.32	&	33.03	&	1.8	&	1.9	&	329	&	5.34	&	...	\\
3FGL J1549.1$-$5347c*	&	15:48:38.12	&	$-$53:44:00.33	&	1.67	&	51.64	&	10.89	&	0.13	&	998.9	&	2.9	&	1172	&	5.27	&	spp	\\
3FGL J1039.1$-$5809	&	10:38:25.85	&	$-$58:08:23.45	&	4.54	&	37.46	&	24.69	&	23.37	&	1.7	&	1.3	&	107	&	5.23	&	...	\\
3FGL J1831.7$-$0230	&	18:31:33.96	&	$-$02:31:25.54	&	1.94	&	31.1	&	17.8	&	2.08	&	17.4	&	2.7	&	421	&	5.23	&	...	\\
3FGL J1702.8$-$5656$^\dagger$	&	17:02:45.00	&	$-$56:54:39.46	&	0.63	&	58.78	&	46.9	&	53.13	&	3.4	&	2.1	&	1917	&	5.19	&	...	\\
3FGL J1736.0$-$2701*	&	17:36:07.44	&	$-$27:03:29.55	&	2.29	&	38.45	&	25.23	&	23.68	&	0.3	&	0.0	&	80	&	5.18	&	...	\\
3FGL J2023.5$+$4126*	&	20:23:24.65	&	$+$41:27:31.08	&	1.45	&	48.95	&	78.1	&	36.72	&	0.4	&	0.0	&	93	&	5.12	&	...	\\
3FGL J1758.8$-$2346	&	17:59:09.58	&	$-$23:47:19.28	&	1.23	&	41.8	&	11.84	&	5.36	&	20.8	&	1.9	&	218	&	5.01	&	...	\\
3FGL J2004.4$+$3338*	&	20:04:22.03	&	$+$33:39:29.46	&	0.49	&	50.29	&	13.47	&	0.03	&	866.5	&	2.4	&	708	&	5.01	&	...	\\
3FGL J0212.1$+$5320$^\dagger$	&	02:12:12.29	&	$+$53:20:49.61	&	0.53	&	51.47	&	45.93	&	82	&	3.3	&	1.5	&	1442	&	5.01	&	...	\\
3FGL J1901.1$+$0728	&	19:01:09.32	&	$+$07:30:01.23	&	1.10	&	55.34	&	25.81	&	10.48	&	6.6	&	2.0	&	134	&	4.88	&	...	\\
3FGL J1503.5$-$5801	&	15:03:39.92	&	$-$58:00:43.22	&	1.29	&	67.48	&	26.29	&	18.7	&	3.7	&	2.0	&	359	&	4.85	&	...	\\
3FGL J1850.5$-$0024	&	18:50:31.56	&	$-$00:24:33.69	&	1.61	&	64.27	&	14.64	&	2.78	&	7.7	&	2.3	&	216	&	4.76	&	...	\\
3FGL J0933.9$-$6232$^\dagger$	&	09:34:00.41	&	$-$62:32:57.43	&	0.59	&	59.2	&	87.95	&	125.91	&	2.0	&	0.8	&	907	&	4.73	&	...	\\
3FGL J1620.0$-$5101	&	16:19:48.66	&	$-$51:00:57.34	&	1.34	&	50.48	&	9.74	&	0.97	&	64.9	&	2.1	&	121	&	4.72	&	...	\\
3FGL J1726.6$-$3530c	&	17:26:32.27	&	$-$35:33:37.61	&	1.73	&	60.31	&	10.99	&	1.76	&	20.2	&	2.6	&	335	&	4.67	&	...	\\
3FGL J1919.9$+$1407	&	19:20:11.19	&	$+$14:11:54.53	&	2.65	&	67.73	&	17.57	&	0.25	&	87.2	&	2.7	&	642	&	4.66	&	...	\\
3FGL J1119.9$-$2204$^\dagger$	&	11:19:59.45	&	$-$22:04:25.17	&	0.60	&	62.62	&	103.18	&	156.94	&	1.7	&	1.3	&	1949	&	4.63	&	...	\\
3FGL J0907.0$-$4802*	&	09:07:18.05	&	$-$47:58:38.32	&	3.37	&	40.75	&	29.27	&	27.97	&	0.4	&	0.2	&	123	&	4.58	&	...	\\
3FGL J1718.0$-$3726	&	17:18:02.10	&	$-$37:26:50.06	&	0.34	&	41.58	&	1.54	&	2.04	&	80.1	&	2.1	&	593	&	4.55	&	snr	\\
3FGL J1859.6$+$0102	&	18:59:39.72	&	$+$01:00:15.56	&	1.81	&	68.61	&	18.88	&	13.08	&	3.5	&	1.8	&	150	&	4.40	&	...	\\
3FGL J2035.0$+$3634	&	20:35:02.11	&	$+$36:32:12.74	&	0.63	&	52.58	&	39.23	&	57.54	&	2.8	&	0.8	&	401	&	4.39	&	...	\\
3FGL J1345.1$-$6224	&	13:44:43.61	&	$-$62:28:30.64	&	1.71	&	58.3	&	12.76	&	1.3	&	29.5	&	2.7	&	568	&	4.39	&	spp	\\
3FGL J0744.1$-$2523$^\dagger$	&	07:44:06.64	&	$-$25:25:17.47	&	0.66	&	61.34	&	40.89	&	55.28	&	3.2	&	1.8	&	666	&	4.27	&	...	\\
3FGL J0426.7$+$5437$^\dagger$	&	04:26:33.79	&	$+$54:35:00.35	&	1.00	&	51.83	&	63.87	&	58.95	&	1.7	&	2.1	&	1235	&	4.27	&	...	\\
3FGL J1539.2$-$3324$^\dagger$	&	15:39:20.23	&	$-$33:24:56.62	&	0.55	&	57.87	&	102.86	&	129.33	&	2.3	&	0.4	&	694	&	4.22	&	...	\\
3FGL J1641.1$-$4619c*	&	16:41:00.45	&	$-$46:19:46.25	&	0.62	&	39.43	&	0.65	&	0.24	&	150.0	&	2.3	&	292	&	4.15	&	spp	\\
\textbf{3FGL J1528.3$-$5836}	&	15:28:23.37	&	$-$58:38:05.98	&	0.62	&	68.72	&	44.89	&	41.41	&	4.0	&	1.6	&	452	&	4.14	&	...	\\
3FGL J1814.1$-$1734c$^\dagger$	&	18:58:03.73	&	$+$03:55:08.04	&	1.69	&	41.47	&	11.17	&	32.18	&	2.2	&	1.4	&	131	&	4.13	&	...	\\
3FGL J1855.4$+$0454	&	18:55:12.72	&	$+$04:55:38.38	&	1.49	&	38.6	&	6.59	&	4.4	&	10.5	&	2.4	&	193	&	4.12	&	...	\\
3FGL J1650.0$-$4438c*	&	16:49:48.42	&	$-$44:38:58.44	&	2.21	&	58.81	&	0.95	&	0.06	&	918.9	&	3.1	&	843	&	4.02	&	...	\\
3FGL J0901.6$-$4700$^\dagger$	&	09:01:40.90	&	$-$46:52:10.77	&	2.34	&	55.1	&	30.04	&	52.65	&	1.0	&	1.2	&	221	&	4.02	&	...	\\
3FGL J1329.8$-$6109	&	13:29:57.92	&	$-$61:08:00.95	&	0.82	&	55.66	&	22.5	&	21.14	&	4.9	&	1.6	&	246	&	3.91	&	...	\\
3FGL J1639.4$-$5146	&	16:39:25.17	&	$-$51:46:04.03	&	0.46	&	58.03	&	4.2	&	2.82	&	46.3	&	2.3	&	945	&	3.85	&	...	\\
3FGL J1833.9$-$0711*	&	18:34:10.57	&	$-$07:11:34.47	&	1.04	&	82.07	&	1.63	&	0.35	&	997.5	&	2.3	&	482	&	3.85	&	spp	\\
3FGL J1814.0$-$1757c	&	18:14:07.87	&	$-$17:36:39.99	&	0.99	&	50.07	&	7.11	&	5.33	&	3.9	&	1.4	&	83	&	3.73	&	...	\\
3FGL J1139.0$-$6244	&	11:39:07.61	&	$-$62:46:04.02	&	0.77	&	29.45	&	7.46	&	16.52	&	8.6	&	1.9	&	278	&	3.71	&	...	\\
3FGL J1626.2$-$2428c	&	16:26:25.40	&	$-$24:31:36.54	&	1.58	&	46.87	&	15.87	&	7.77	&	7.8	&	2.1	&	392	&	3.66	&	...	\\
3FGL J1212.2$-$6251	&	12:12:18.06	&	$-$62:53:31.51	&	0.95	&	53.7	&	1.4	&	12.9	&	45.8	&	2.4	&	426	&	3.45	&	spp	\\

\tablecomments{List of 3FGL sources searched for gamma-ray pulsars using Einstein@Home, ranked by their probability to be pulsars according to the GMM analysis presented in Section~\ref{s:classification}. Sources marked with a $\dagger$ symbol were searched in a previous Einstein@Home \& \textit{Atlas} survey for gamma-ray pulsars. Sources for which suspiciously low or high cutoff energies were measured are marked with an asterisk. We highlighted in bold face the 3FGL sources in which pulsars were discovered in this survey. The discovery and analysis of PSRs J1906+0722 and J1208$-$6238 are presented in \citet{Clark2015ApJJ1906} and \citet{ClarkJ1208}, while PSRs J1035$-$6720 and PSR J1744$-$7619 discovered in 3FGL~J1035.7$-$6720 and 3FGL~J1744.1$-$7619 will be presented in a future publication. Columns 2 to 4 list the searched positions and radii. Columns 5 and 6 give the variability and curvature indices VI and $\textrm{TS}_\textrm{curve}$ from the 3FGL catalog. Columns 7 to 10 give the curvature TS values, the cutoff energies and the photon indices from our binned maximum likelihood analysis with \texttt{Pointlike}. Column is the logritmic of pulsar likelihood calculate from GMM. Column 12 lists association flags from the 3FGL catalog. ``pwn'' and ``snr'' labels indicate possible associations with pulsar wind nebulae (PWN) and supernova remnants (SNR) respectively, sources with class ``spp'' are special cases with potential PWN or SNR associations. Sources below the horizontal line were searched with the re-locatized position mentioned in \ref{s:reloc}. }

%\tablecomments{The source list sorted with the logarithmic likelihood from GMM. Sources with $\dagger$ were searched in previous Einstein@Home/Altas blind search survey. Sources with ``*'' means the spectral fit result in abnormal value. Columns 2 - 4 list the searched posistion and the radius of the search region covered. Columns 5 and 6 list the cataloged VI and $TS_{curve}$ from the 3FGL catalog. Columns 7$-$10 are the spectral parameters result from the binned likelihood analysis with Pointlike. Column 10 is the source assiocation flag taken from the 3FGL catalog, ``pwn'' and ``snr'' represent possible assiocation with pulsar wind nebula (PWN) and supernova remnant (SNR) respectivity, sources with class ``spp'' are special case indicates potential assoication with SNR or PWN.}

\enddata
	
\end{deluxetable*}


